If in a Crowdsourced Data Annotation Pipeline, a GPT-4

Recent studies indicated GPT-4 outperforms online crowd workers in data labeling accuracy, notably workers from Amazon Mechanical Turk (MTurk). However, these studies were criticized for deviating from standard crowdsourcing practices and emphasizing individual workers' performances over the whole data-annotation process. This paper compared GPT-4 and an ethical and well-executed MTurk pipeline, with 415 workers labeling 3,177 sentence segments from 200 scholarly articles using the CODA-19 scheme. Two worker interfaces yielded 127,080 labels, which were then used to infer the final labels through eight label-aggregation algorithms. Our evaluation showed that despite best practices, MTurk pipeline's highest accuracy was 81.5%, whereas GPT-4 achieved 83.6%. Interestingly, when combining GPT-4's labels with crowd labels collected via an advanced worker interface for aggregation, 2 out of the 8 algorithms achieved an even higher accuracy (87.5%, 87.0%). Further analysis suggested that, when the crowd's and GPT-4's labeling strengths are complementary, aggregating them could increase labeling accuracy.

==> Sections/2-2-Crowd-AI-data-annotation.tex <==
% Before GPT, there were several works being explored to help annotator to label data. 

==> Tables/agree_disagree/One-Coin.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\setlength{\tabcolsep}{2.8pt}
\begin{tabular}{llrrrrrrrrrrrrrrrrrr}
\toprule
\multicolumn{1}{l}{\textbf{Eval}} & \multicolumn{3}{c}{\textbf{Background}} & \multicolumn{3}{c}{\textbf{Purpose}} & \multicolumn{3}{c}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Finding}} & \multicolumn{3}{c}{\textbf{Other}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Acc}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Kappa}}} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16}
% \cline{2-16}
\textbf{Label} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\ \midrule
\multicolumn{19}{c}{\textbf{Basic UI} \textit{All-Workers}} \\
Agree (pure crowd)  & .909 & .503 & .647 & .389 & .659 & .489 & .531 & .807 & .641 & .884 & .789 & .834 & 1.000 & .308 & .471 & .723 & .583 \\
Disagree (pure crowd)  & .429 & .129 & .199 & .068 & .156 & .095 & .335 & .452 & .385 & .315 & .353 & .333 & 1.000 & .125 & .222 & .295 & .044 \\
Agree (crowd + gpt)  & .936 & .789 & .856 & .624 & .762 & .686 & .737 & .912 & .815 & .944 & .894 & .918 & .857 & .462 & .600 & .865 & .792 \\
Disagree (crowd + gpt)  & .603 & .317 & .415 & .143 & .313 & .196 & .412 & .504 & .453 & .341 & .353 & .347 & 1.000 & .125 & .222 & .380 & .156 \\
\multicolumn{19}{c}{\textbf{Basic UI} \textit{Exclude-By-Worker}} \\
Agree (pure crowd)  & .875 & .538 & .667 & .423 & .665 & .517 & .546 & .798 & .649 & .880 & .798 & .837 & 1.000 & .308 & .471 & .733 & .596 \\
Disagree (pure crowd)  & .420 & .151 & .222 & .101 & .219 & .139 & .328 & .437 & .375 & .293 & .323 & .307 & 1.000 & .125 & .222 & .293 & .038 & \\
Agree (crowd + gpt)  & .934 & .814 & .870 & .634 & .778 & .699 & .756 & .917 & .829 & .950 & .896 & .922 & .857 & .462 & .600 & .874 & .806 \\
Disagree (crowd + gpt)  & .614 & .367 & .459 & .139 & .344 & .198 & .400 & .459 & .428 & .349 & .338 & .344 & 1.000 & .125 & .222 & .380 & .161 \\
\multicolumn{19}{c}{\textbf{Basic UI} \textit{Exclude-By-Batch}} \\
Agree (pure crowd)  & .892 & .503 & .643 & .357 & .654 & .462 & .518 & .813 & .632 & .896 & .763 & .825 & 1.000 & .308 & .471 & .710 & .569 \\
Disagree (pure crowd)  & .410 & .115 & .180 & .093 & .250 & .136 & .310 & .452 & .367 & .306 & .286 & .296 & 1.000 & .125 & .222 & .277 & .028 \\
Agree (crowd + gpt)  & .936 & .805 & .865 & .633 & .773 & .696 & .743 & .919 & .822 & .949 & .891 & .919 & .857 & .462 & .600 & .869 & .799 \\
Disagree (crowd + gpt)  & .595 & .338 & .431 & .149 & .344 & .208 & .398 & .489 & .439 & .339 & .323 & .331 & 1.000 & .125 & .222 & .376 & .152 \\
\multicolumn{19}{c}{\textbf{Advanced UI} \textit{All-Workers}} \\
Agree (pure crowd)  & .724 & .465 & .566 & .165 & .584 & .257 & .443 & .730 & .551 & .923 & .528 & .672 & .000 & .000 & .000 & .557 & .397 \\
Disagree (pure crowd)  & .423 & .158 & .230 & .049 & .219 & .080 & .387 & .533 & .449 & .354 & .173 & .232 & .000 & .000 & .000 & .277 & .064 \\
Agree (crowd + gpt)  & .953 & .948 & .951 & .752 & .870 & .807 & .868 & .967 & .915 & .983 & .927 & .954 & 1.000 & .462 & .632 & .933 & .898 \\
Disagree (crowd + gpt)  & .707 & .590 & .643 & .098 & .250 & .140 & .547 & .600 & .572 & .510 & .368 & .428 & .800 & .500 & .615 & .501 & .328 \\
\multicolumn{19}{c}{\textbf{Advanced UI} \textit{Exclude-By-Worker}} \\
Agree (pure crowd)  & .914 & .852 & .881 & .694 & .686 & .690 & .756 & .928 & .834 & .947 & .897 & .922 & 1.000 & .385 & .556 & .877 & .811 \\
Disagree (pure crowd)  & .652 & .432 & .519 & .082 & .219 & .120 & .474 & .548 & .509 & .451 & .383 & .415 & 1.000 & .125 & .222 & .432 & .234 \\
Agree (crowd + gpt)  & .950 & .961 & .956 & .774 & .886 & .826 & .879 & .963 & .919 & .983 & .929 & .955 & 1.000 & .462 & .632 & .937 & .904 \\
Disagree (crowd + gpt)  & .708 & .612 & .656 & .103 & .281 & .151 & .539 & .563 & .551 & .511 & .361 & .423 & .800 & .500 & .615 & .497 & .324 \\
\multicolumn{19}{c}{\textbf{Advanced UI} \textit{Exclude-By-Batch}} \\
Agree (pure crowd)  & .732 & .485 & .583 & .178 & .605 & .275 & .459 & .752 & .570 & .928 & .545 & .687 & .000 & .000 & .000 & .575 & .419 \\
Disagree (pure crowd)  & .426 & .144 & .215 & .061 & .281 & .101 & .402 & .548 & .464 & .420 & .218 & .287 & .000 & .000 & .000 & .295 & .089 \\
Agree (crowd + gpt)  & .950 & .953 & .952 & .764 & .876 & .816 & .871 & .969 & .917 & .984 & .926 & .955 & 1.000 & .538 & .700 & .935 & .900 \\
Disagree (crowd + gpt)  & .712 & .604 & .654 & .119 & .313 & .172 & .545 & .585 & .564 & .510 & .368 & .428 & .750 & .375 & .500 & .503 & .331 \\
\midrule
Agree gpt-4  & .896 & .968 & .930 & .637 & .903 & .747 & .837 & .961 & .895 & .996 & .833 & .907 & .295 & 1.000 & .456 & .892 & .839 \\
Disagree gpt-4  & .701 & .691 & .696 & .152 & .500 & .234 & .493 & .504 & .498 & .673 & .263 & .378 & .400 & .750 & .522 & .494 & .334 \\
 \bottomrule

% gpt-4 (t=1.0)  & .820 & .920 & .867 & .493 & .829 & .619 & .766 & .876 & .818 & .978 & .789 & .874 & .365 & .241 & .290 & .930 & .780 \\
% CS Expert  & .863 & .821 & .841 & .541 & .853 & .662 & .856 & .801 & .828 & .911 & .921 & .916 & 1 & .165 & .283 & \textbf{.940} & .814 \\ \hline
\end{tabular}
\caption{}
% \steven{aggregation with 20 labels}
\label{table:one-coin-agree-disagree-stats}
\end{table}

==> Tables/gpt-improvement-example-1-pretty-exclude-worker-one-coin.tex <==
\begin{table}[t]
\centering \small
\begin{tabular}{llp{7.5cm}ccc}
    \toprule
    \textbf{Index} & \textbf{C/I} & \textbf{Sentence Sample} & \textbf{Gold Label} & \textbf{GPT} & \textbf{Crowd+GPT} \\ \midrule
    1 & \textbf{C}   & There were also some differences due to adaptation to online conferences , & Finding & Method & Finding \\  \hline
    2 & \textbf{C} & allow us to provide health strategies with more intelligent capabilities to accurately predict the outcomes of the disease in daily life and the hospital and prevent the progression of this disease and its many complications . & Method & Purpose & Method \\ \hline
    3 & \textbf{C}   & CONCLUSION : Regarding all initial variables , & Finding & Other & Finding \\  \hline
    4 & \textbf{C}   & Most participants were female ( 68 \% ) , & Finding & Method & Finding \\  \hline
    5 & \textbf{C}   & 4.5 M ) in Canada , & Finding & Other & Finding \\  \hline
    6 & \textbf{C}   & and examine associations longitudinally to better understand causality . & Finding & Purpose & Finding \\  \hline
    7 & \textbf{C}   & and financial strain may be mutually reinforcing and compound the health consequence of smoking . & Finding & Background & Finding \\  \hline
    8 & \textbf{C} & SUMMARY : This article summarizes the components of the healthcare maintenance visit for CMC , & Finding & Purpose & Finding \\ \hline
    9 & \textbf{I}   & there is no evidence of transmission of coronavirus COVID-19 by tick as a vector • To date , & Finding & Finding & Background \\ 
    
    \bottomrule
\end{tabular}
\caption{Ground Truth (Bio Expert) Label Stats Summary}
\label{table:gpt-improvement-example-1}
\end{table}



==> Tables/ground-truth-label-summary.tex <==
\begin{table*}[t]

\centering \small
\begin{tabular}{cccccc}
    \toprule
     \textbf{All Labels} & \textbf{Background} & \textbf{Purpose} & \textbf{Method} & \textbf{Finding} & \textbf{Other} \\ \midrule
     3,177 & 698 & 217 & 680 & 1,561 & 21 \\ \bottomrule
\end{tabular}
\caption{Ground Truth (Bio Expert) Label Stats Summary}
\label{table:ground-truth-label-summary}
\end{table*}
